Scan2Part: Fine-grained and Hierarchical Part-level Understanding of Real-World 3D Scans

We propose Scan2Part, a method to segment individual parts of objects in real-world, noisy indoor RGB-D scans. To this end, we vary the part hierarchies of objects in indoor scenes and explore their effect on scene understanding models. Specifically, we use a sparse U-Net-based architecture that captures the fine-scale detail of the underlying 3D scan geometry by leveraging a multi-scale feature hierarchy. In order to train our method, we introduce the Scan2Part dataset, which is the first large-scale collection providing detailed semantic labels at the part level in the real-world setting. In total, we provide 242,081 correspondences between 53,618 PartNet parts of 2,477 ShapeNet objects and 1,506 ScanNet scenes, at two spatial resolutions of 2 cm$^3$ and 5 cm$^3$. As output, we are able to predict fine-grained per-object part labels, even when the geometry is coarse or partially missing.

==> src/fig/fig_dataset_anno_percentage.tex <==
\begin{figure}[h]
\label{fig:dataset_anno_percent}
\centering
\includegraphics[width=0.48\textwidth]{img/anotated_voxels_number.png}
\caption{Percentage of annotated voxels vs. distance to ground truth surface.}
\end{figure}


==> src/fig/fig_dataset_construction_label_transfer.tex <==
\begin{figure*}[!h]
\centering
\includegraphics[width=0.9\textwidth]{img/scan2part_labels_transfer}
\caption{An overview of our pipeline for part-based 3D scan annotation. 
Our method for obtaining fine-grained part-level labels is fully automatic and free of manual labour.}
\label{fig:dataset_schema}
\end{figure*}



==> src/pre.tex <==
\twocolumn[{
\vspace{-3em}
\maketitle
\vspace{-3em}
% \begin{@twocolumnfalse}
% \begin{center}
% \includegraphics[width=0.8\textwidth]{example-image-golden}
% \captionof{figure}{test caption}
% \end{center}
% % \begin{figure}
% % \caption{x}
% \label{fig:teaser}
% % \end{figure}
% \end{@twocolumnfalse}
}]
